Non-Wellfounded and Cyclic Proofs for LTL: A Syntactic Correspondence with Linear Nested Sequents

We introduce the formalism of non-wellfounded and cyclic linear nested sequent calculi, developing concrete systems for linear temporal logic (LTL). The paper addresses two central problems, which we call "cycle recognition" and "unraveling." Cycle recognition concerns identifying cycles in non-wellfounded proofs in order to extract corresponding cyclic proofs, while unraveling studies the converse transformation, from cyclic proofs to non-wellfounded ones. Although these processes are well understood for Gentzen sequents, they have received little attention for more expressive sequent formalisms and become more challenging in the linear nested sequent setting. To address cycle recognition, we show the completeness of non-wellfounded proofs relative to a particular normal form exhibiting a property we call "saturation recurrence," which enables the systematic extraction of cyclic proofs. To address unraveling, we introduce a specialized procedure that shifts rule applications forward along linear nested sequents, allowing non-wellfounded proofs to be reconstructed from cyclic ones. Overall, our work provides new proof-theoretic techniques for cycle recognition and unraveling in expressive multisequent formalisms.

==> Storage.tex <==
\begin{proof} We prove the invertibility of all non-initial rules in $\calci$ by a simultaneous coinduction. We only consider cases where the $\untillii$ rule is to be inverted as the argument for other rules is analogous. Therefore, we assume that we have a non-wellfounded proof $\prf$ of $\lnsg \sslash \Gamma, A \until B \sar \Delta$. We make a case distinction on the last rule applied in $\prf$. We consider a representative number of cases.

$\id$. Let $\prf$ be the proof shown below left. Then, we can obtain proofs $\prf_{1}$ and $\prf_{2}$ of the corresponding premises of $\untillii$, shown below middle and below right, respectively.
\begin{center}
\begin{tabular}{c c c}
\AxiomC{$\phantom{\lnsg}$}
\RightLabel{$\id$}
\UnaryInfC{$\lnsg \sep \Gamma', p, A \until B \sar p, \Delta'$}
\DisplayProof

&

\AxiomC{$\phantom{\lnsg}$}
\RightLabel{$\id$}
\UnaryInfC{$\lnsg \sep \Gamma', p, B \sar p, \Delta'$}
\DisplayProof

&

\AxiomC{$\phantom{\lnsg}$}
\RightLabel{$\id$}
\UnaryInfC{$\lnsg \sep \Gamma', p, A \sar p, \Delta' \sslash A \until B \sar$}
\DisplayProof
\end{tabular}
\end{center}
The case where the principal formulas of $\id$ occur in a different component is analogous.

$\untillii$. There are two cases to consider. % if $\prf$ ends with $\untillii$. 
If $A \until B$ is principal, then the proofs $\prf_{1}$ and $\prf_{2}$ of both premises give the desired proofs. Suppose then that $A \until B$ is not principal in $\untillii$, as shown below. 
\begin{center}
\begin{tabular}{c}
\AxiomC{$\dotprf{\prf_{1}}$}
\UnaryInfC{$\lnsg \sep \Gamma', D, A \until B \sar \Delta$}

\AxiomC{$\dotprf{\prf_{2}}$}
\UnaryInfC{$\lnsg \sep \Gamma', C, A \until B \sar \Delta \sep C \until D \sar $}
\RightLabel{$\untillii$}
\BinaryInfC{$\lnsg \sep \Gamma', C \until D, A \until B \sar \Delta$}
\DisplayProof
\end{tabular}
\end{center}
By the coinduction hypothesis for $\untillii$, we have proofs $\prf_{1}'$ of $\lnsg \sep \Gamma', D, B \sar \Delta$ and $\prf_{1}''$ of $\lnsg \sep \Gamma', D, A \sar \Delta \sslash A \until B \sar $. By the coinduction hypothesis for $\untilli$, we have proofs $\prf_{2}'$ of $\lnsg \sep \Gamma', C, B \sar \Delta \sep C \until D \sar $ and $\prf_{2}''$ of $\lnsg \sep \Gamma', C, A \sar \Delta \sep C \until D, A \until B \sar $. We obtain a non-wellfounded proof $\prf''$ of the right premise of $\untillii$ as shown below.
\begin{center}
\AxiomC{$\dotprf{\prf_{1}''}$}
\UnaryInfC{$\lnsg \sep \Gamma', D, A \sar \Delta \sslash A \until B \sar $}

\AxiomC{$\dotprf{\prf_{2}''}$}
\UnaryInfC{$\lnsg \sep \Gamma', C, A \sar \Delta \sep C \until D, A \until B \sar $}
\RightLabel{$\untilli$}
\BinaryInfC{$\lnsg \sep \Gamma', C \until D, A \sar \Delta \sslash A \until B \sar $}
\DisplayProof
\end{center}
The proof $\prf'$ for the left premise is obtained similarly, using the proofs $\prf_{1}'$ and $\prf_{2}'$ with %an application of 
$\untillii$.


$\untilri$. Let $\prf$ be the non-wellfounded proof shown below. We consider the case where an auxiliary component of $\untilri$ is the same as the principal component of $\untillii$. By the coinduction hypothesis, we have non-wellfounded proofs $\prf_{1}'$ of $\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, B \sar \Delta$, $\prf_{1}''$ of $\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar$, $\prf_{2}'$ of $\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, B \sar C \until D, \Delta$, and $\prf_{2}''$ of $\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \sar C \until D, \Delta \sslash A \until B \sar $. 
\begin{center}
\AxiomC{$\dotprf{\prf_{1}}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \until B \sar \Delta$}
\AxiomC{$\dotprf{\prf_{2}}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \until B \sar C \until D, \Delta$}
\RightLabel{$\untilri$}
\BinaryInfC{$\lnsg \sep \Sigma \sar C \until D, \Pi \sep \Gamma, A \until B \sar \Delta$}
\DisplayProof
\end{center}
We obtain a non-wellfounded proof $\prf''$ of the right premise of $\untillii$ as shown below.
\begin{center}
\AxiomC{$\dotprf{\prf_{1}''}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar$}
\AxiomC{$\dotprf{\prf_{2}''}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \sar C \until D, \Delta \sslash A \until B \sar $}
\RightLabel{$\untilri$}
\BinaryInfC{$\lnsg \sep \Sigma \sar C \until D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar $}
\DisplayProof
\end{center}
The proof $\prf'$ for the left premise is obtained similarly, using proofs $\prf_{1}'$ and $\prf_{2}'$ with an application of $\untilri$.

$\nextlii$. Let $\prf$ be the non-wellfounded proof shown below left. By the coinduction hypothesis for $\untilli$ we have a non-wellfounded proof $\prf_{1}'$ of $\lnsg \sep \Gamma, B \sar \Delta \sep C \sar $ and $\prf_{1}''$ of $\lnsg \sep \Gamma, A \sar \Delta \sep A \until B, C \sar $. The desired non-wellfounded proofs $\prf'$ and $\prf''$ can be obtained as shown below middle and below right, respectively.
\begin{center}
\begin{tabular}{c c c}
\AxiomC{$\dotprf{\prf_{1}}$}
\UnaryInfC{$\lnsg \sep \Gamma, A \until B \sar \Delta \sep C \sar $}
\RightLabel{$\nextlii$}
\UnaryInfC{$\lnsg \sep \Gamma, A \until B, \X C \sar \Delta$}
\DisplayProof

&

\AxiomC{$\dotprf{\prf_{1}'}$}
\UnaryInfC{$\lnsg \sep \Gamma, B \sar \Delta \sep C \sar $}
\RightLabel{$\nextlii$}
\UnaryInfC{$\lnsg \sep \Gamma, B, \X C \sar \Delta$}
\DisplayProof

&

\AxiomC{$\dotprf{\prf_{1}''}$}
\UnaryInfC{$\lnsg \sep \Gamma , A \sar \Delta \sep A \until B, C \sar $}
\RightLabel{$\nextli$}
\UnaryInfC{$\lnsg \sep \Gamma, A, \X C \sar \Delta \sslash A \until B \sar $}
\DisplayProof
\end{tabular}
\end{center}
This concludes the proof of the lemma.
\end{proof}






$\untilri$. Let $\prf$ be the non-wellfounded proof shown below. We consider the case where an auxiliary component of $\untilri$ is the same as the principal component of $\untillii$. By the coinduction hypothesis, we have non-wellfounded proofs $\prf_{1}'$ of $\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, B \sar \Delta$, $\prf_{1}''$ of $\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar$, $\prf_{2}'$ of $\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, B \sar C \until D, \Delta$, and $\prf_{2}''$ of $\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \sar C \until D, \Delta \sslash A \until B \sar $. 
\begin{center}
\AxiomC{$\dotprf{\prf_{1}}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \until B \sar \Delta$}
\AxiomC{$\dotprf{\prf_{2}}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \until B \sar C \until D, \Delta$}
\RightLabel{$\untilri$}
\BinaryInfC{$\lnsg \sep \Sigma \sar C \until D, \Pi \sep \Gamma, A \until B \sar \Delta$}
\DisplayProof
\end{center}
We obtain a non-wellfounded proof $\prf''$ of the right premise of $\untillii$ as shown below.
\begin{center}
\AxiomC{$\dotprf{\prf_{1}''}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar C, D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar$}
\AxiomC{$\dotprf{\prf_{2}''}$}
\UnaryInfC{$\lnsg \sep \Sigma \sar D, \Pi \sep \Gamma, A \sar C \until D, \Delta \sslash A \until B \sar $}
\RightLabel{$\untilri$}
\BinaryInfC{$\lnsg \sep \Sigma \sar C \until D, \Pi \sep \Gamma, A \sar \Delta \sslash A \until B \sar $}
\DisplayProof
\end{center}
The proof $\prf'$ for the left premise is obtained similarly, using proofs $\prf_{1}'$ and $\prf_{2}'$ with an application of $\untilri$.

$\nextlii$. Let $\prf$ be the non-wellfounded proof shown below left. By the coinduction hypothesis for $\untilli$ we have a non-wellfounded proof $\prf_{1}'$ of $\lnsg \sep \Gamma, B \sar \Delta \sep C \sar $ and $\prf_{1}''$ of $\lnsg \sep \Gamma, A \sar \Delta \sep A \until B, C \sar $. The desired non-wellfounded proofs $\prf'$ and $\prf''$ can be obtained as shown below middle and below right, respectively.
\begin{center}
\begin{tabular}{c c c}
\AxiomC{$\dotprf{\prf_{1}}$}
\UnaryInfC{$\lnsg \sep \Gamma, A \until B \sar \Delta \sep C \sar $}
\RightLabel{$\nextlii$}
\UnaryInfC{$\lnsg \sep \Gamma, A \until B, \X C \sar \Delta$}
\DisplayProof

&

\AxiomC{$\dotprf{\prf_{1}'}$}
\UnaryInfC{$\lnsg \sep \Gamma, B \sar \Delta \sep C \sar $}
\RightLabel{$\nextlii$}
\UnaryInfC{$\lnsg \sep \Gamma, B, \X C \sar \Delta$}
\DisplayProof

&

\AxiomC{$\dotprf{\prf_{1}''}$}
\UnaryInfC{$\lnsg \sep \Gamma , A \sar \Delta \sep A \until B, C \sar $}
\RightLabel{$\nextli$}
\UnaryInfC{$\lnsg \sep \Gamma, A, \X C \sar \Delta \sslash A \until B \sar $}
\DisplayProof
\end{tabular}
\end{center}
This concludes the proof of the lemma.









\begin{proof} 
Let $\lnsg$ be the conclusion of a rule $\mathsf{r}$ of $\calci$ and let $\lnsh$ be one of the premises. Suppose $\pi$ is a proof of $\lnsg$. We first show how to define a derivation of $\lnsh$ by coinduction on $\pi$. We consider the cases where $\mathsf{r} \in \{{\to} \mathsf{R}, \untillii\}$. The other cases are argued similarly and omitted. \smallskip

\noindent \textsc{Case for ${\to} \mathsf{R}$.} Suppose $\pi$ is a non-wellfounded proof of $\lnsg \sep \Gamma \vdash A \to B, \Delta \sep \lnsh$. We show how to construct a derivation $h(\pi)$ of the premise $\lnsg \sep \Gamma, A \vdash B, \Delta \sep \lnsh$ by coinduction. We make a case distinction on the last rule applied in $\prf$.



$\id$. Suppose $\pi$ is the proof depicted below.
\begin{scprooftree}{1}
\AxiomC{$\phantom{\lnsg}$}
\RightLabel{$\id$}
\UnaryInfC{$\lnsg_0 \sep \Sigma, p \sar p, \Pi \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
\end{scprooftree}
Define $h(\pi)$ to be
\begin{scprooftree}{1}
\AxiomC{$\phantom{\lnsg}$}
\RightLabel{$\id$}
\UnaryInfC{$\lnsg_0 \sep \Sigma, p \sar p, \Pi \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
\end{scprooftree}
The case where the axiom occurs in a different component is similar. Moreover, the case where the last rule applied in $\pi$ is ${\bot}\mathsf{L}$ is similar as well. 

${\to}\mathsf{R}$. There are two cases to consider. First suppose that the formula $A \to B$ is principal in ${\to}\mathsf{R}$, i.e. $\pi$ is of the following form, where $\pi_0$ is the proof of the premise.
\begin{prooftree}
    \AxiomC{$\pi_0$}
    \noLine
    \UnaryInfC{$\lnsg \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
    \RightLabel{${\to}\mathsf{R}$}
    \UnaryInfC{$\lnsg \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
\end{prooftree}
Then define $h(\pi) := \pi_0$. Otherwise a different formula $C \to D$, potentially in a different component, is principal, i.e. $\pi$ is of the following form.
\begin{prooftree}
    \AxiomC{$\pi_0$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma, C \sar D, \Pi \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
    \RightLabel{${\to}\mathsf{R}$}
    \UnaryInfC{$\lnsg_0 \sep \Sigma \sar C \to D, \Pi \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
\end{prooftree}
Then define $h(\pi)$ to be the following derivation.
\begin{prooftree}
    \AxiomC{$h(\pi_0)$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma, C \sar D, \Pi \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
    \RightLabel{${\to}\mathsf{R}$}
    \UnaryInfC{$\lnsg_0 \sep \Sigma \sar C \to D, \Pi \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
\end{prooftree}
where $h(\pi_0)$ is obtained by coinductively applying the transformation to $\pi_0$. The cases where the principal formula occurs in a different component are treated analogously. The cases where the last rule applied in $\pi$ is $\mathsf{r} \in \{{\to}\mathsf{L},\nextli, \nextlii, \nextri, \nextrii, \untilli, \untillii, \untilri, \untilrii\}$ are all treated similarly. We only discuss the case for $\untilli$.

$\untilli$. Suppose the last rule applied in $\pi$ is $\untilli$ with principal formula $C \until D$.
\begin{scprooftree}{0.85}
    \AxiomC{$\pi_0$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma_0, D \sar \Pi_0 \sep \Sigma_1 \sar \Pi_1 \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
    \AxiomC{$\pi_1$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma_0, C \sar \Pi_0 \sep \Sigma_1, C \until D \sar \Pi_1 \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
    \RightLabel{$\untilli$}
    \BinaryInfC{$\lnsg_0 \sep \Sigma_0, C \until D\sar \Pi_0 \sep \Sigma_1 \sar \Pi_1 \sep \lnsg_1 \sep \Gamma \sar A \to B, \Delta \sep \lnsh$}
\end{scprooftree}
Then define $h(\pi)$ to be the following derivation.
\begin{scprooftree}{0.85}
    \AxiomC{$h(\pi_0)$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma_0, D \sar \Pi_0 \sep \Sigma_1 \sar \Pi_1 \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
    \AxiomC{$h(\pi_1)$}
    \noLine
    \UnaryInfC{$\lnsg_0 \sep \Sigma_0, C \sar \Pi_0 \sep \Sigma_1, C \until D \sar \Pi_1 \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
    \RightLabel{$\untilli$}
    \BinaryInfC{$\lnsg_0 \sep \Sigma_0, C \until D\sar \Pi_0 \sep \Sigma_1 \sar \Pi_1 \sep \lnsg_1 \sep \Gamma, A \sar B, \Delta \sep \lnsh$}
\end{scprooftree}
The case where the principal formula is in a different component is similar. This finishes the case where $\mathsf{r} = {\to}\mathsf{R}$. \smallskip

\noindent \textsc{Case for $\untillii$.} Suppose $\pi$ is a non-wellfounded proof of $\lnsg \sep \Gamma, A \until B \sar \Delta$. We show how to construct proofs $h_0(\pi)$ of the left premise $\lnsg \sep \Gamma, B \sar \Delta$ and $h_1(\pi)$ of the right premise $\lnsg \sep \Gamma, A \sar \Delta \sep A \until B \sar $ of $\untillii$ by coinduction. We make a case distinction on the last rule applied in $\pi$. We consider the cases where the last rule applied is $\untillii$, $\untilri$ and $\nextlii$. All other cases are argued similarly.

$\untillii$. There are two cases to consider. First suppose that $A \until B$ is principal in $\untillii$, i.e. $\pi$ is of the following form.
\begin{prooftree}
    \AxiomC{$\pi_0$}
    \noLine
    \UnaryInfC{$\lnsg \sep \Gamma, B \sar \Delta$}
    \AxiomC{$\pi_1$}
    \noLine
    \UnaryInfC{$\lnsg \sep \Gamma, A \sar \Delta \sep A \until B \sar$}
    \RightLabel{$\untillii$}
    \BinaryInfC{$\lnsg \sep \Gamma, A \until B \sar \Delta$}
\end{prooftree}
Then define $h_0(\pi) := \pi_0$ and $h_1(\pi) := \pi_1$. Second, suppose that $A \until B$ is not principal in $\untillii$. Then $\pi$ is of the following form.
\begin{prooftree}
\AxiomC{$\pi_0$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', D, A \until B \sar \Delta$}
\AxiomC{$\pi_1$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', C, A \until B \sar \Delta \sep C \until D \sar $}
\RightLabel{$\untillii$}
\BinaryInfC{$\lnsg \sep \Gamma', C \until D, A \until B \sar \Delta$}
\end{prooftree}
Define $h_0(\pi)$ to be the following derivation.
\begin{prooftree}
\AxiomC{$h_0(\pi_0)$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', D, B \sar \Delta$}
\AxiomC{$h_0(\pi_1)$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', C, B \sar \Delta \sep C \until D \sar $}
\RightLabel{$\untillii$}
\BinaryInfC{$\lnsg \sep \Gamma', C \until D, B \sar \Delta$}
\end{prooftree}
Moreover, define $h_1(\pi)$ to be the following derivation.
\begin{prooftree}
\AxiomC{$h_1(\pi_0)$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', D, A \sar \Delta \sslash A \until B \sar $}
\AxiomC{$h_1(\pi_1)$}
\noLine
\UnaryInfC{$\lnsg \sep \Gamma', C, A \sar \Delta \sep C \until D, A \until B \sar $}
\RightLabel{$\untilli$}
\BinaryInfC{$\lnsg \sep \Gamma', C \until D, A \sar \Delta \sslash A \until B \sar $}
\end{prooftree}

\end{proof}


We call a rule \emph{admissible} in a proof system if, whenever its premises have proofs, its conclusion also has a proof.\footnote{We define a \emph{proof} to be either a non-wellfounded proof or cyclic proof.} Given an $n$-ary rule $\ru$, we let $\ru^{-1}_{i}$ denote its \emph{$i$-inverse}, obtained by taking the conclusion of $\ru$ as the premise and the $i^\text{th}$ premise as the conclusion. $\ru$ is \emph{invertible} \iffi $\ru^{-1}_{i}$ is admissible for each $1 \leq i \leq n$. 




For soundness, due to the presence of infinite branches, a more complicated argument than an induction on the height of proofs is required. Instead we argue by contradiction and assume that some invalid LNS $\lnsg$ has a non-wellfounded proof $\pi$. Since $\lnsg$ is invalid, there exists a state sequence $\model$ such that $\model, 0 \not \models \lnsg$. We then show how to obtain a branch $\branch =\{\lnsg_i\}_{i\in \mathbb{N}}$ of $\pi$ such that $\model, 0 \not\models \lnsg_i$ for each $i \in \mathbb{N}$, by showing that all rules of $\calci$ are locally sound, i.e., that if the conclusion is invalid, then at least some premise is invalid. Note that $\branch$ must be an infinite branch of $\pi$, since initial sequents are always valid. Simultaneously, we assign to each trace value occurring in an LNS along $\branch$ a well-founded measure and show that for any trace pair $(\bracket{A \until B, j}, \bracket{A \until B, k})$ occurring in $\branch$ the measure strictly decreases when the trace pair is progressing and weakly decreases otherwise. Finally, since $\pi$ is a proof, $\branch$ must contain a suffix with a progressing trace. By construction, the measure along this trace never increases and strictly decreases infinitely often, which contradicts the fact that the measure is well-founded. This gives the desired contradiction and thus soundness of $\calci$.

\begin{theorem}[Soundness of $\calci$]\label{thm:soundness}
    If $\calci \proves \lnsk$, then $\lnsk$ is valid.
\end{theorem}
\begin{proof}
    Let $\pi$ be a $\calci$-proof of $\lnsk$ and suppose, for contradiction, that $\lnsk$ is not valid. Then there exists a state sequence $\model$ such that $\model, 0 \not \models \lnsk$. We will inductively define an infinite path of LNSs $(\lnsk_i)_i$ through $\pi$ and an infinite sequence of maps $(\mu_i)_i$ such that for all $i \in \mathbb{N}$ the following hold:
    \begin{enumerate}
        \item $\model, 0 \not \models \lnsk_i$;
        \item $\mu_i$ is a signature for $\lnsk_i$;
        \item for every trace value $\bracket{A \until B,j}$ of $\lnsk_i$ the following hold:
        \begin{enumerate}
            \item $\mu_i(\bracket{A \until B,j})$ is the least natural number $k$ such that $\model, j+k \models B$ and for each $0 \leq k' < k$ holds $\model, j+k' \models A$;
            \item if $(\bracket{A \until B,j}, \bracket{A \until B,j})$ is a trace pair for $(\lnsk_{i-1}, \lnsk_{i})$, then $\mu_{i}(\bracket{A \until B,j}) \leq \mu_{i-1}(\bracket{A \until B,j})$;
            \item if $(\bracket{A \until B,j}, \bracket{A \until B,j+1})$ is a trace pair for $(\lnsk_{i-1}, \lnsk_{i})$, then $\mu_{i}(\bracket{A \until B,j+1}) < \mu_{i-1}(\bracket{A \until B,j})$.
        \end{enumerate}
    \end{enumerate}
    We define $(\lnsk_i)_i$ and $(\mu_i)_i$ as follows. Let $\lnsk_0 := \lnsk$. Since $\model, 0 \not \models \lnsk$, we have $\model, j \models A \until B$ for each trace value $\bracket{A \until B, j}$ of $\lnsk$. Therefore there exists a natural number $k$ such that (i) $\model, j + k \models B$, and (ii) $\model, j + k' \models A$ for each $0 \leq k' < k$. Hence let $\mu_0$ be the map that assigns to each trace value $\bracket{A \until B, j}$ of $\lnsk$ the least natural number $k$ such that (i) and (ii) hold. Note that 1--3 are satisfied.

    Suppose we have defined $\lnsk_i$ and $\mu_i$ and they satisfy 1--3. We define $\lnsk_{i+1}$ and $\mu_{i+1}$ by using a case distinction based on the rule $\mathsf{r}$ with conclusion $\lnsk_i$ in $\pi$. Note that $\mathsf{r}$ cannot be an initial rule, since $\model, 0 \not \models \lnsk_i$ by 1. We show the case for $\untilli$; the other cases are argued similarly. Suppose $\lnsk_i$ is the conclusion of an instance of $\untilli$, as shown below.
    \begin{center}
\begin{tabular}{c}
\AxiomC{$\overbrace{\lnsg \sep \Gamma, B \sar \Delta \sep \Sigma \sar \Pi \sep \lnsh}^{\lnsk'}$}
\AxiomC{$\overbrace{\lnsg \sep \Gamma, A \sar \Delta \sep \Sigma, A \until B  \sar \Pi \sep \lnsh}^{\lnsk''}$}
\RightLabel{$\untilli$}
\BinaryInfC{$\underbrace{\lnsg \sep \Gamma, A \until B \sar \Delta \sep \Sigma \sar \Pi \sep \lnsh}_{\lnsk_i}$}
\DisplayProof
\end{tabular}
\end{center}

Suppose $\Gamma, A \until B \sar \Delta$ is the $j$-component of $\lnsk_i$ and the principal formula forms the trace value $\bracket{A \until B, j}$ of $\lnsk_i$. If $\mu_i(\bracket{A \until B, j}) = 0$, then $\model, j \models B$. Hence let $\lnsk_{i+1} = \lnsk'$ and observe that $\model, 0 \not \models \lnsk_{i+1}$. If $B=C \until D$ for some formulae $C,D$, then let $\mu_{i+1}(\bracket{B,j})$ be the least natural number $k$ which satisfies that $\model, j+k \models D$ and $\model, j+k' \models C$ for all $0 \leq k' < k$. For any other trace value $\bracket{C \until D, l}$ of $\lnsk_{i+1}$, note that $(\bracket{C \until D, l}, \bracket{C \until D, l})$ is a trace pair for $(\lnsk_i, \lnsk_{i+1})$. Therefore let $\mu_{i+1}(\bracket{C \until D, l}) = \mu_i(\bracket{C \until D, l})$. Note that 1--3 are satisfied.

If $\mu_i(\bracket{A \until B, j}) > 0$, then observe that $\model, j \models A$ and $\model, j+1 \models A \until B$ by 3(a). Hence let $\lnsk_{i+1} = \lnsk''$ and note that $\model, 0 \not \models \lnsk_{i+1}$. If $A=C \until D$ for some formulae $C,D$, then let $\mu_{i+1}(\bracket{A,j})$ be the least natural number $k$ which satisfies that $\model, j+k \models D$ and $\model, j+k' \models C$ for all $0 \leq k' < k$. Furthermore, let $\mu_{i+1}(\bracket{A \until B, j+1}) = \mu_i(\bracket{A \until B, j}) - 1$. For any other trace value $\bracket{E \until F, l}$ of $\lnsk_{i+1}$, note that $(\bracket{E \until F, l}, \bracket{E \until F, l})$ is a trace pair for $(\lnsk_i, \lnsk_{i+1})$. Therefore let $\mu_{i+1}(\bracket{E \until F, l}) = \mu_i(\bracket{E \until F, l})$. Note that 1--3 are satisfied. This concludes the construction of $(\lnsk_i)_i$ and of $(\mu_i)_i$.

Since $\pi$ is a proof, the infinite branch $(\lnsk_i)_i$ must have a suffix $\lnspath= (\lnsk_i)_{i \geq j}$ that is a progressing path. Hence there exists a progressing trace $(\tau_i)_{i \geq j}$ along $\lnspath$. Consider the infinite sequence of natural numbers $(\mu_i(\tau_i))_{i\geq j}$. By 3(b) and 3(c) we have that for each $i \geq j$, $\mu_{i+1}(\tau_{i+1}) \leq \mu_i(\tau_i)$. Since the trace is progressing, there are infinitely many progressing trace pairs $(\tau_i, \tau_{i+1})$, so 3(c) implies that there are infinitely many $i \geq j$ with $\mu_{i+1}(\tau_{i+1}) < \mu_i(\tau_i)$. Therefore $(\mu_i(\tau_i))_i$ is a decreasing sequence of natural numbers which is strictly decreasing infinitely often. This contradicts the wellfoundedness of natural numbers. Hence $\lnsk$ is valid. 
\end{proof}







%%%%%%%%%%Shifting Lemma%%%%%%%%%%

\begin{lemma}[Shifting Lemma]\label{lem:shifting}
Let $\tuple{\der,L,c}$ be a cyclic proof of $\lnsg$ with $\lnsg = c(\lnsg')$ and $\lnsg' \in L$. Then, there exists a strictly isomorphic cyclic proof $\tuple{\der',L',c'}$ of $\lnsg'$.
\end{lemma}

\begin{proof} Let $\lnsg = \lnsh \sslash \Gamma \sar \Delta$ and $\lnsg' = \lnsh \sslash \lnsk \sslash \Gamma \sar \Delta$ such that $\size{\lnsk} \geq 1$, $\size{\lnsg} = n$, and $\size{\lnsg'} = k$. By definition, $\lnsg$ and $\lnsg'$ are saturated. We simultaneously define a derivation $\pi'$ of $\lnsg'$ and a strict isomorphism $\shift$ from LNSs in $\prf$ to LNSs in $\pi'$ in a stepwise manner. We refer to $\prf$ as the `input proof' and to $\prf'$ as the `output proof'. We show by induction on the depth $d$ of $\lnsf$ in $\prf$ that the following invariant (I) holds, which is a conjunction of three statements: (a) $h$ is an isomorphism up to depth $d$, (b) $\lnsf$ is saturated \iffi $\shift(\lnsf)$ is saturated, and (c) if $i \geq n$, then $\lnsf(i) = \shift(\lnsf)(j)$ with $j = k + (i - n)$.

We remark that condition (c) ensures that components at or
beyond the index $n$ in LNSs of the input proof are preserved
via $h$ in the output proof, but shifted forward by $(k - n)$
positions. This shift reflects the fact that $\lnsg'$ extends $\lnsg$ with the additional components of $\lnsk$. Moreover, since $\lnsg$ is saturated, rule applications in the input proof are confined to $i$-components with $i \geq n$, and these are precisely the components that are relocated from the index $i$ to the index $k + (i - n)$ in the output.


\case{Base case.} We let the derivation of $\lnsg'$ be the tree consisting of the single node $\lnsg'$ and set $\shift(\lnsg) := \lnsg'$. Note that (I) holds by the shape of $\lnsg$ and $\lnsg'$.

%\case{Inductive step.}We make a case distinction on the rule applied to $\lnsf$ in $\prf$. We show the $\impr$ and $\untilrii$ cases as the remaining cases are similar. Observe that rule applications are confined to $i$-components such that $i \geq n$ due to the fact that $\lnsg$ is saturated, i.e., no complex formulae appear in $\lnsh$.

\case{Inductive step.} We make a case distinction on the rule applied to $\lnsf$ in $\prf$. We show the $\impr$ and $\untilrii$ cases as the remaining cases are similar. As noted above, since $\lnsg$ is saturated, all rule applications occur at $i$-components with $i \geq n$.


\case{Case for $\impr$.}Suppose $\impr$ is applied bottom-up (shown below left) to the $i$-component of $\lnsf$ in $\prf$ with $d$ the depth of $\lnsf$ in $\prf$. By IH, we have constructed the output derivation and map $\shift$ up to depth $d$ and know that the $i$-component of $\lnsf$ is equal to the $j$-component of $\shift(\lnsf)$. We extend the output derivation by bottom-up applying $\impr$ to the $j$-component of $\shift(\lnsf)$, as shown below right.
\begin{center}
\begin{tabular}{c c}
\AxiomC{$\lnsf\set{\Sigma, A \sar B, \Pi}_{i}$}
\RightLabel{$\impr$}
\UnaryInfC{$\lnsf\set{\Sigma \sar A \imp B, \Pi}_{i}$}
\DisplayProof

&

\AxiomC{$\shift(\lnsf)\set{\Sigma, A \sar B, \Pi}_{j}$}
\RightLabel{$\impr$}
\UnaryInfC{$\shift(\lnsf)\set{\Sigma \sar A \imp B, \Pi}_{j}$}
\DisplayProof
\end{tabular}
\end{center}
We set $\shift(\lnsf\set{\Sigma, A \sar B, \Pi}_{i}) := \shift(\lnsf)\set{\Sigma, A \sar B, \Pi}_{j}$. For all $m \neq i$ with $m \geq n$, the $m$-component has been unaffected by the $\impr$ application, so the $m$-component of $\lnsf\set{\Sigma, A \sar B, \Pi}_{i}$ and the $k+(m-n)$-component of $\shift(\lnsf)\set{\Sigma, A \sar B, \Pi}_{j}$ are equal. Also, observe that the $i$-component of $\lnsf\set{\Sigma, A \sar B, \Pi}_{i}$ is equal to the $j$-component of $\shift(\lnsf)\set{\Sigma, A \sar B, \Pi}_{j}$. This implies that (c) holds and, moreover, that $\lnsf\set{\Sigma, A \sar B, \Pi}_{i}$ is saturated iff $\shift(\lnsf)\set{\Sigma, A \sar B, \Pi}_{j}$. Therefore, (I) holds between both premises above.

\case{Case for $\untilrii$.} Let $\untilrii$ be applied bottom-up to the $i$-component of $\lnsf$ with $d$ the depth of $\lnsf$ in $\prf$.
\begin{center}
\AxiomC{$\lnsf\set{\Sigma \sar A, B, \Pi}_{i}$}
\AxiomC{$\lnsf\set{\Sigma \sar B, \Pi \sep \sar A \until B}_{i}$}
\RightLabel{$\untilrii$}
\BinaryInfC{$\lnsf\set{\Sigma \sar A \until B, \Pi}_{i}$}
\DisplayProof
\end{center}
By IH, we know that the $i$-component of $\lnsf$ is equal to the $j$-component of $\shift(\lnsf)$, and so, we may bottom-up apply $\untilrii$ to the $j$-component of $\shift(\lnsf)$, as shown below.
\begin{center}
\AxiomC{$\shift(\lnsf)\set{\Sigma \sar A, B, \Pi}_{j}$}
\AxiomC{$\shift(\lnsf)\set{\Sigma \sar B, \Pi \sep \sar A \until B}_{j}$}
\RightLabel{$\untilrii$}
\BinaryInfC{$\shift(\lnsf)\set{\Sigma \sar A \until B, \Pi}_{j}$}
\DisplayProof
\end{center}
By an argument similar to the $\impr$ case, one can verify that (I) holds between the premises of the above rule applications. This concludes the definition of $\shift$.

We now show that $\pi'$ is a cyclic proof of $\lnsg'$ that is weakly isomorphic to $(\pi, L, c)$. First, note that by construction $h$ is a weak isomorphism between $\pi$ and $\pi'$. Let $(c(\lnsf),\lnsf)$ form a cycle in $(\prf, L, c)$. By the definition of $\shift$, we know that a path occurs from $\shift(c(\lnsf))$ to $\shift(\lnsf)$ in $\prf'$ with $h(\lnsf)$ a leaf of $\pi'$ and that since $\size{c(\lnsf)} < \size{\lnsf}$, the path from $c(\lnsf)$ to $\lnsf$ passes through an expansion rule and so the path from $h(c(\lnsf))$ to $h(\lnsf)$ passes through an expansion rule as well, implying that $\size{h(c(\lnsf))} < \size{h(\lnsf)}$. Moreover, by the invariant (I), we know that $h(\lnsf)$ and $h(c(\lnsf))$ are saturated since $\lnsf$ and $c(\lnsf)$ are saturated, $\last{\lnsf} = \last{h(\lnsf)}$, and $\last{c(\lnsf)} = \last{h(c(\lnsf))}$. Therefore, since $\last{c(\lnsf)} = \last{\lnsf}$, we have $\last{h(c(\lnsf))} = \last{h(\lnsf)}$. Since $(c(\lnsf), \lnsf)$ is a cycle in a cyclic proof, the path from $c(\lnsf)$ to $\lnsf$ has a continuous focus trace that passes through the right premise of a rule $\ru \in \set{\untilli,\untillii}$ with the formula in focus principal. By construction of $h$ and (I), the path from $h(c(\lnsf))$ to $h(\lnsf)$ therefore has a continuous focus trace that passes through the right premise of a rule $\ru \in \set{\untilli,\untillii}$ with the formula in focus principal. Let $L' := \set{h(\lnsf) \mid \lnsf \in L}$ and let $c'$ map each $h(\lnsf) \in L'$ to $h(c(\lnsf))$. For any other leaf $h(\lnsh)$ of $\pi'$, $\lnsh$ is a leaf of $\pi$ which does not belong to $L$ and therefore is an initial sequent. By (I), $h(\lnsh)$ is an initial sequent as well; therefore, $(\pi', L', c')$ is a cyclic proof of $\lnsg'$ that is weakly isomorphic to $(\pi, L,c)$.
\end{proof}

==> sec-admiss-normal-forms.tex <==



\begin{figure*}[t]
%\noindent\hrule

\begin{center}
\begin{tabular}{c c c}
\AxiomC{$\lnsg \sep \Gamma \sar \Delta \sep \lnsh$}
\RightLabel{$\wk$}
\UnaryInfC{$\lnsg \sep \Gamma, \Sigma \sar \Pi, \Delta \sep \lnsh$}
\DisplayProof

&

\AxiomC{$\lnsg \sep \Gamma \sar \Delta \sep \Sigma \sar \Pi$}
\RightLabel{$\ew$}
\UnaryInfC{$\lnsg \sep \lnsk \sep \Gamma \sar \Delta \sep \Sigma \sar \Pi$}
\DisplayProof

&

\AxiomC{$\lnsg \sep \Gamma \sar \Delta$}
\RightLabel{$\chop$}
\UnaryInfC{$\Gamma \sar \Delta$}
\DisplayProof
\end{tabular}
\end{center}

\smallskip

\begin{center}
\begin{tabular}{c c}
\AxiomC{$\lnsg \sep \Gamma, \phi, \phi \sar \Delta \sep \lnsh$}
\RightLabel{$\ctrl$}
\UnaryInfC{$\lnsg \sep \Gamma, \phi \sar \Delta \sep \lnsh$}
\DisplayProof

&

\AxiomC{$\lnsg \sep \Gamma \sar \phi, \phi, \Delta \sep \lnsh$}
\RightLabel{$\ctrr$}
\UnaryInfC{$\lnsg \sep \Gamma \sar \phi, \Delta \sep \lnsh$}
\DisplayProof
\end{tabular}
\end{center}


%\noindent\rule{38em}{0.4pt}
\caption{TODO.\label{fig:calc}}
\end{figure*}


\begin{lemma}
The weakening rule $\wk$ is admissible in $\calci$.
\end{lemma}

\begin{proof}
TODO
\end{proof}

\begin{lemma}
The contraction rules $\ctrl$ and $\ctrr$ are admissible in $\calci$.
\end{lemma}



\begin{lemma}
The external weakening rule $\ew$ is end-active admissible in $\calci$.
\end{lemma}



\begin{lemma}
The trim rule $\chop$ is end-active admissible in $\calci$.
\end{lemma}





\begin{definition}[Splice~\cite{KuzLel18}] Let $\lnsg$ and $\lnsh$ be linear nested sequents. We define the \emph{splice} $\lnsg \otimes \lnsh$ by recursion on the length of both $\lnsg$ and $\lnsh$ as shown below:
\begin{flalign*}
& (\Gamma \vdash \Delta) \otimes (\Sigma \vdash \Pi)  :=  \Gamma, \Sigma \vdash \Delta, \Pi &&\\
& (\Gamma \vdash \Delta) \otimes (\Sigma \vdash \Pi \sslash \lnsk)  :=  \Gamma, \Sigma \vdash \Delta, \Pi \sslash \lnsk &&\\
& (\Gamma \vdash \Delta \sslash \lnsk) \otimes (\Sigma \vdash \Pi)  :=  \Gamma, \Sigma \vdash \Delta, \Pi \sslash \lnsk &&\\
& (\Gamma \vdash \Delta \sslash \lnsk) \otimes (\Sigma \vdash \Pi \sslash \lnsf)  :=  \Gamma, \Sigma \vdash \Delta, \Pi \sslash (\lnsk \otimes \lnsf) &&
\end{flalign*}
\end{definition}


\begin{theorem}[Cut-Elimination]\label{thm:cut-elim}
The $\cut$ rule is admissible in $\calci$, where $\seqlen{\lnsg} = \seqlen{\lnsk}$.
\begin{center}
\AxiomC{$\lnsg \sep \Gamma \sar \phi, \Delta \sep \lnsh$}
\AxiomC{$\lnsk \sep \Sigma, \phi \sar \Pi \sep \lnsf$}
\RightLabel{$\cut$}
\BinaryInfC{$(\lnsg \otimes \lnsk) \sep \Gamma, \Sigma \sar \Delta, \Pi \sep (\lnsh \otimes \lnsf)$}
\DisplayProof
\end{center}
\end{theorem}



==> sec-sound-compl.tex <==

In this section, we remark the soundness and completeness of $\calci$. In the subsequent section, we will define mutual proof transformations between non-wellfounded and cyclic proofs, yielding soundness and completeness of $\calccyc$ as a corollary.

To establish soundness of $\calci$ we argue by contradiction and assume that some invalid LNS $\lnsg$ has a non-wellfounded proof $\pi$. Since $\lnsg$ is invalid, there exists a state sequence $\model$ such that $\model \not \sat \lnsg$. We then show how to obtain a branch $\branch =\{\lnsg_i\}_{i\in \mathbb{N}}$ of $\pi$ such that $\model \not\sat \lnsg_i$ for each $i \in \mathbb{N}$, by using that all rules of $\calci$ are locally sound (see Lemma~\ref{lem: local soundness}). Note that $\branch$ must be an infinite branch of $\pi$, since initial sequents are always valid. Simultaneously, we assign a well-founded measure in the form of natural numbers to annotated formulae occurring in LNSs along $\branch$ and show that whenever a formula $A \until B^\an$ is principal in $\untilli$ or $\untillii$ and $\branch$ passes through the right premise, the measure assigned to $A \until B^\an$ strictly decreases, and weakly decreases otherwise. Finally, since $\pi$ is a proof, $\branch$ must contain a progressing suffix, meaning that there is a stable annotation $\an$ and the suffix passes infinitely often through the right premise of instances of $\untilli$ and $\untillii$ with the formula annotated by $\an$ principal. Thus we obtain an infinite decreasing sequence of natural numbers which strictly decreases infinitely often, which contradicts that natural numbers are well-founded. This gives the desired contradiction and thus soundness of $\calci$. The full proof can be found in Appendix~\ref{app:soundness}.

\begin{theorem}[Soundness of $\calci$]\label{thm:soundness}
    If $\calci \proves \lnsg$, then $\lnsg$ is valid.
\end{theorem}

Completeness of $\calci$ is established by a proof-search argument. Given an LNS $\lnsg$, we show how to build a derivation $\pi$, called a \emph{proof-search tree}, such that either $\pi$ is a non-wellfounded proof of $\lnsg$ or we can construct a counter-model of $\lnsg$ from a `bad' branch of $\pi$. For the purposes of translating non-wellfounded into cyclic proofs, we construct the proof-search tree such that it satisfies the  %to obtain completeness with respect to proofs that satisfy a certain saturation principle. Namely, a derivation $\pi$ satisfies the 
\emph{saturation recurrence property} (SRP): a derivation $\pi$ satisfies the SRP if and only if, for any infinite branch $\branch := \{\lnsg_i\}_{i \in \mathbb{N}}$ in $\pi$, infinitely many $\lnsg_i$ are saturated. %In the following we will thus show that if an LNS $\lnsg$ is valid, then it has an $\calci$-proof which satisfies the SRP.
Therefore we obtain the following result. The full proof is shown in Appendix~\ref{app:completeness}.

\iffalse
We call $\nextlii$, $\nextrii$, $\untillii$ and $\untilrii$ \emph{expansion} rules and all other logical rules \emph{length-preserving}. An LNS $\lnsg$ is called \emph{fully saturated} \iffi for $0 \leq i < \size{\lnsg}$, $\lnsg$ is $i$-saturated, i.e., $\lnsg$ is not the conclusion of any instance of a rule in $\calci$. We formalize proof-search by means of \emph{proof-search trees} which represent a systematic search for a proof of a given LNS. 

\begin{definition} A \emph{proof-search tree} for an LNS $\lnsg$ is a derivation $\pi$ of $\lnsg$ such that the following hold:
\begin{enumerate}

\item[$(1)$] Every rule instance in $\pi$ is succinct;

\item[$(2)$] The conclusion of every instance of an expansion rule is saturated;

\item[$(3)$] Every leaf of $\pi$ is an initial sequent or a fully saturated sequent.

\end{enumerate}
\end{definition}


Intuitively, given an LNS $\lnsg$, we obtain a proof-search tree by applying length-preserving rules bottom-up until every leaf is either an initial sequent or saturated. Branches ending in initial sequents or fully saturated leaves are closed, while branches ending in saturated leaves that are \emph{not fully saturated} are extended by bottom-up applying an expansion rule. Since the premise of an expansion rule may no longer be saturated, this process can be repeated. We thus obtain the following lemma, whose proof is standard and omitted.


\begin{lemma}
    Every LNS $\lnsg$ has a proof-search tree.
\end{lemma}

Since in a proof-search tree every rule is applied succinctly and expansion rules are only applied to saturated LNSs, a simple inductive argument shows that every infinite branch tree contains infinitely many saturated sequents and so that every proof-search tree satisfies the SRP. The proof of the following lemma is deferred to Appendix~\ref{app:completeness}.
 
\begin{lemma}\label{lem: SRP}
    Let $\lnsg$ be an LNS and $\pi$ be a proof-search tree for $\lnsg$. Then, $\pi$ satisfies the SRP.
\end{lemma}


Observe that if $\branch=\set{\lnsg_i}_{i \in \mathbb{N}}$ is an infinite branch of a proof-search tree $\pi$, then there are infinitely many $i \in \mathbb{N}$ such that $\size{\lnsg_i} < \size{\lnsg_{i+1}}$, since $\pi$ satisfies the SRP and rules are applied succinctly. In particular if $\lnsg_i$ is saturated and the conclusion of an instance of $\untilrii$ with $\lnsg_{i+1}$ the left premise, then $\lnsg_{i+1}$ is saturated and its size does not grow. However, since the instance is succinct and sequents are ordered pairs of \emph{finite} sets of annotated formulae, this situation can only occur finitely many times before $\branch$ passes through an expansion rule that does increase the size of the premise. We now show that every LNS has an $\calci$-proof which satisfies the SRP or is falsifiable, from which completeness readily follows.

\begin{lemma}\label{lem: proof or falsifiable}
    Let $\lnsg$ be an LNS. Then, $\lnsg$ has an $\calci$-proof which satisfies the SRP or there exists a state sequence $\Bar{\sigma}$ such that $\Bar{\sigma} \not \sat \lnsg$.
\end{lemma}
\begin{proof}
    Let $\lnsg$ be an LNS and let $\pi$ be a proof-search tree for $\lnsg$. Recall that $\pi$ is a derivation. If $\pi$ is a proof, then $\lnsg$ has an $\calci$-proof which satisfies the SRP by Lemma~\ref{lem: SRP}. Otherwise $\pi$ contains a `bad' branch $\branch$: either $\branch$ is finite and ends in a fully saturated sequent or $\branch$ is infinite and not progressing. We only consider the latter case, as the former is argued similarly. 

    So suppose $\branch := \set{\lnsg_{i}}_{i \in \mathbb{N}}$ is an infinite branch of $\der$ which is \emph{not} progressing. We use the branch $\branch$ to construct a state sequence $\sts$ such that $\sts \not\sat \lnsg$. Let us define:
$$
\Gamma_{i} := \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \bigcup_{j \in \mathbb{N}, \, \lnsg_{j}(i) \, = \, (\Gamma \, \sar \, \Delta)} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \Gamma
\qquad
\Delta_{i} := \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \bigcup_{j \in \mathbb{N}, \, \lnsg_{j}(i) \, = \, (\Gamma \, \sar \, \Delta)} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \Delta
$$
We define $\sigma_{i} = \set{p \mid p \in \Gamma_{i}}$ and $\bar\sigma=\tuple{\sigma_0,\sigma_1,\ldots}$. We now prove the following by a mutual induction on the length of $A$: (1) if $A^\an \in \Gamma_{i}$ for an annotation $\an$, then $\sts, i \sat A$ and (2) if $A^\an \in \Delta_{i}$ for an annotation $\an$, then $\sts, i \not\sat A$. We consider the case for $A = B \until C$. The full proof is shown in Appendix~\ref{app:completeness}.

%\case{Case for $A = \bot \in \Gamma_i$.}By definition there exists a $j$ such that $\bot \in \lnsg_j(i)$. Therefore $\lnsg_j$ is an initial sequent, and so, by definition of a proof-search tree, the branch $\branch$ ends in $\lnsg_j$. This gives a contradiction, and therefore $\bot \not \in \Gamma_i$.

%\case{Case for $A = \bot \in \Delta_i$.}By definition $\model, i \not \models \bot$.

%\case{Case for $A = p \in \Gamma_{i}$.}By definition $p \in \sigma_{i}$, therefore $\sts, i \sat p$.

%\case{Case for $A = p \in \Delta_{i}$.}Suppose towards a contradiction that $p \in \Gamma_{i}$ as well. Then, there are $j_0,j_1$ with  $\lnsg_{j_0}(i) = \Sigma \sar \Pi$ and $\lnsg_{j_1}(i) = \Sigma' \sar \Pi'$, such that $p \in \Sigma$ and $p \in \Pi'$. Suppose without loss of generality that $j_0 \leq j_1$. By definition of the rules of $\calci$, note that $p \in \Sigma$ implies that $p \in \Sigma'$, since there are no rules that delete atoms. Therefore, $p \in \Sigma' \cap \Pi'$ and so $\lnsg_{j_1}$ is an instance of $\id$. By definition of a proof-search tree, the branch $\branch$ ends in $\lnsg_{j_1}$. This gives a contradiction, and so, $p \not\in \Gamma_{i}$, meaning, $\sts, i \not \sat p$.

%\case{Case for $A=B \to C \in \Delta_i$.}By definition, there exists a $j$ such that $B \to C \in \Pi$ with $\lnsg_j(i) = \Sigma \sar \Pi$. Since $\pi$ satisfies the SRP, there exists $k > j$ such that $\lnsg_k$ is saturated and $\size{\lnsg_{j}} < \size{\lnsg_{k}}$. This implies that in the segment of $\branch$ between $\lnsg_j$ and $\lnsg_k$ there is an instance of ${\to}\mathsf{R}$ with $B \to C$ principal. Hence, for some $j \leq l \leq k$ with $\lnsg_l(i)=\Sigma' \sar \Pi'$ we have $B \in \Sigma'$ and $C \in \Pi'$ and so $B \in \Gamma_i$ and $C \in \Delta_i$. By IH, $\Bar{\sigma}, i \sat B$ and $\Bar{\sigma}, i \not \sat C$, implying that $\Bar{\sigma}, i \not \sat B \to C$. The case for $A=B \to C \in \Gamma_i$ is similar and omitted. %By definition, there exists a $j$ such that $B \to C \in \Pi$ with $\lnsg_j(i) = \Sigma \sar \Pi$. We distinguish two cases. (1) Suppose $\size{\lnsg_j} > i+1$ (i.e., $\Sigma \sar \Pi$ is not the end component). Since $\pi$ satisfies the SRP, there exists $k > j$ such that $\lnsg_k$ is saturated. This implies that in the segment of $\branch$ between $\lnsg_j$ and $\lnsg_k$ there is an instance of ${\to}\mathsf{R}$ with $B \to C$ principal. Hence for some $j \leq l \leq k$ with $\lnsg_l(i)=\Sigma' \sar \Pi'$ we have $B \in \Sigma'$ and $C \in \Pi'$ and so $B \in \Gamma_i$ and $C \in \Delta_i$. By IH $\Bar{\sigma}, i \sat B$ and $\Bar{\sigma}, i \not \sat C$, implying that $\Bar{\sigma}, i \not \sat B \to C$. (2) Suppose $\size{\lnsg_j}=i+1$. Then, $B \to C$ occurs in the end component of $\lnsg_j$. Since $\pi$ satisfies the SRP, there exists a least $k \geq j$ such that $\lnsg_k$ is saturated. If there exists an instance of ${\to}\mathsf{R}$ with $B \to C$ principal in the segment from $\lnsg_j$ to $\lnsg_k$, then $\Bar{\sigma}, i \not \sat B \to C$ follows by the same argument as before. Otherwise, by definition of a proof-search tree, $\lnsg_k$ is the conclusion of an instance of an expansion rule, implying that $\size{\lnsg_{k+1}} = i+2$ and so that $B \to C$ is not in the end component of $\lnsg_{k+1}$. Case (1) then implies that $\Bar{\sigma}, i \not \sat B \to C$. The case for $A=B \to C \in \Gamma_i$ is similar and omitted.

%\case{Case for $A = \X B \in \Gamma_{i}$.}By definition, there exists a $j$ such that $\X B \in \Sigma$ with $\lnsg_{j}(i) = \Sigma \sar \Pi$. Since $\pi$ satisfies the SRP, there exists a natural number $k > j$ such that $\lnsg_k$ is saturated and $\size{\lnsg_{j}} < \size{\lnsg_{k}}$. This implies that in the segment of $\branch$ between $\lnsg_j$ and $\lnsg_k$ there is an instance of the rule $\nextli$ or $\nextlii$ with $\X B$ principal. Hence, for some $j \leq l \leq k$ with $\lnsg_l(i+1) = \Sigma' \sar \Pi'$ we have $B \in \Sigma'$, and so $B \in \Gamma_{i+1}$. By IH, it follows that $\sts, i+1 \sat B$, meaning, $\sts, i \sat \X B$. The case for $A=\X B \in \Delta_i$ is similar and omitted. %By definition, there exists a $j$ such that $\X B \in \Sigma$ with $\lnsg_{j}(i) = \Sigma \sar \Pi$. We distinguish two cases. (1) Suppose $\size{\lnsg_j} > i+1$. Since $\pi$ satisfies the SRP, there exists a natural number $k > j$ such that $\lnsg_k$ is saturated. This implies that in the segment of $\branch$ between $\lnsg_j$ and $\lnsg_k$ there is an instance of the rule $\nextli$ with $\X B$ principal. Hence for some $j \leq l \leq k$ with $\lnsg_l(i+1) = \Sigma' \sar \Pi'$ we have $B \in \Sigma'$, and so $B \in \Gamma_{i+1}$. By IH, it follows that $\sts, i+1 \sat B$, meaning, $\sts, i \sat \X B$. (2) Suppose $\size{\lnsg_j} = i+1$. Then $\X B$ occurs in the end component of $\lnsg_j$. Again, since $\pi$ satisfies the SRP, there exists a least $k \geq j$ such that $\lnsg_k$ is saturated. By definition of a proof-search tree, $\lnsg_k$ is the conclusion of an instance of an expansion rule. If this rule is $\nextlii$ with $\X B$ principal, then $B \in \Sigma'$ for $\lnsg_{k+1}(i+1) = \Sigma' \sar \Delta'$ and so $B \in \Gamma_{i+1}$. The IH then implies that $\Bar{\sigma},i+1 \sat B$ and so $\Bar{\sigma},i \sat \X B$. Otherwise $\X B$ is a side formula in the rule instance with $\lnsg_k$ as conclusion. Since an expansion rule is applied, the sequent $\lnsg_{k+1}$ has $i+2$ components, i.e. $\X B$ is not in the end component of $\lnsg_{k+1}$. Case (1) then implies that $\Bar{\sigma}, i \sat \X B$. The case for $A=\X B \in \Delta_i$ is similar and omitted.

\case{Case for $A = B \until C^\an \in \Gamma_{i}$.}By definition, there exists a $j$ such that $B \until C^\an \in \Sigma$ with $\lnsg_{j}(i) = \Sigma \sar \Pi$.  Since $\pi$ satisfies the SRP, there exists an instance of $\untilli$ or $\untillii$ with $B \until C^\an$ principal and $B,C$ and $B \until C^\anb$ residual, where $\anb = \an$ in case $\an \not = \epsilon$. Moreover, since $\branch$ is not progressing, there exists a natural number $k \geq 1$ such that $\untilli$ and $\untillii$ are applied $k$ times above $\lnsg_j$ in the branch $\branch$ such that (1) $B \until C^\anb$ is principal in each instance, (2) for $k-1$ applications, the branch $\branch$ goes through the right premise of $\untilli$ or $\untillii$, and (3) for the $k^\text{th}$ application, the branch $\branch$ goes through the left premise of $\untilli$ or $\untillii$. Otherwise, by the SRP, the path starting at $\lnsg_j$ would have a stable annotation, namely $\anb$, and the path would pass infinitely often through the right premise of $\untilli$ or $\untillii$ with $B \until C^\anb$ principal, which would imply that the path and thus the branch is progressing. Therefore, for $0 \leq n < k-1$, we have $B \in \Gamma_{i+n}$ and $C \in \Gamma_{i+k-1}$. By IH, $\sts, i+n \sat B$ and $\sts, i+k-1 \sat C$, which implies that $\sts, i \sat B \until C$.

\case{Case for $A = B \until C \in \Delta_{i}$.}By definition, there exists a $j$ such that $B \until C \in \Pi$ with $\lnsg_{j}(i) = \Sigma \sar \Pi$. There are two cases to consider. First, it could be the case that $\untilri$ and $\untilrii$ are applied infinitely often above $\lnsg_{j}$ along $\branch$ with $B \until C$ principal and with $\branch$ always going through the right premise of $\untilri$ or $\untilrii$. In this case, we have that $C \in \Delta_{k}$ for all $k \geq i$. By IH, we have that $\sts, k \not\sat C$ for all $k \geq i$, meaning, $\sts, i \not\sat B \until C$. Second, it could be the case that $\untilri$ and $\untilrii$ are applied $k \geq 1$ times\footnote{We note that $k > 0$ since $\pi$ satisfies the SRP by the same argument as before.} above $\lnsg_{j}$ in the branch $\branch$ such that $B \until C$ is principal, the branch $\branch$ goes through the right premise of $\untilri$ or $\untilrii$ for $k-1$ applications, and the branch $\branch$ goes through the left premise of $\untilri$ or $\untilrii$ for the $k^\text{th}$ application. Therefore, for $0 \leq n < k-1$, we have $C \in \Delta_{i+n}$ and $B,C \in \Delta_{i+k-1}$. By IH, $\sts, i+n \not\sat C$, $\sts, i+k-1 \not\sat B$, and $\sts, i+k-1 \not\sat C$, which implies that $\sts, i \not\sat B \until C$.

Finally, let $\lnsg(i) = \Sigma_{i} \sar \Pi_{i}$ for $0 \leq i < \size{\lnsg}$. As $\Sigma_{i} \subseteq \Gamma_{i}$ and $\Pi_{i} \subseteq \Delta_{i}$ for $0 \leq i < \size{\lnsg}$, it follows that $\sts, i \not\sat \lnsg(i)$ for all $0 \leq i < \size{\lnsg}$. Hence, by Definition~\ref{def: satisfaction LNS}, it follows that $\Bar{\sigma} \not \sat \lnsg$ as claimed.
\end{proof}
\fi

\begin{theorem}[Completeness of $\calci$]\label{thm:completeness-non-wf}
If $\lnsg$ is valid, then $\lnsg$ has an $\calci$-proof satisfying the SRP.
\end{theorem}
\iffalse
\begin{proof}
    Suppose $\lnsg$ is valid and let $\pi$ be a proof-search tree for $\lnsg$. By Lemma~\ref{lem: proof or falsifiable}, $\pi$ is either a proof of $\lnsg$ which satisfies the SRP or $\lnsg$ is falsifiable. Since $\lnsg$ is valid, $\lnsg$ is not falsifiable, and so $\pi$ is a proof of $\lnsg$ satisfying the SRP.
\end{proof}
\fi
